MGARD+: Optimizing Multilevel Methods for Error-bounded Scientific Data Reduction

Data management is becoming increasingly important in dealing with the large amounts of data produced by large-scale scientific simulations and instruments. Existing multilevel compression algorithms offer a promising way to manage scientific data at scale, but may suffer from relatively low performance and reduction quality. In this paper, we propose MGARD+, a multilevel data reduction and refactoring framework drawing on previous multilevel methods, to achieve high-performance data decomposition and high-quality error-bounded lossy compression. Our contributions are four-fold: 1) We propose a level-wise coefficient quantization method, which uses different error tolerances to quantize the multilevel coefficients. 2) We propose an adaptive decomposition method which treats the multilevel decomposition as a preconditioner and terminates the decomposition process at an appropriate level. 3) We leverage a set of algorithmic optimization strategies to significantly improve the performance of multilevel decomposition/recomposition. 4) We evaluate our proposed method using four real-world scientific datasets and compare with several state-of-the-art lossy compressors. Experiments demonstrate that our optimizations improve the decomposition/recomposition performance of the existing multilevel method by up to 70X, and the proposed compression method can improve compression ratio by up to 2X compared with other state-of-the-art error-bounded lossy compressors under the same level of data distortion.

==> tex/preamble.tex <==
\usepackage{amsmath, amsthm, mathtools, bm} % math
    \newtheorem{theorem}{Theorem}
\usepackage{graphicx, xcolor}               % graphics
    \definecolor{BLUE}{rgb}{.0, .2, .6}
    \definecolor{BLUEalt}{HTML}{1e50a2}
    % \definecolor{REDalt}{HTML}{c9171e}
    \definecolor{RED}{HTML}{D7003A}
\usepackage{url, hyperref}                  % hyperlink
\usepackage{adjustbox}                      % box
\usepackage{booktabs, multirow}             % table
\usepackage{caption, subcaption}            % caption
    \captionsetup[algorithm]{font=footnotesize}
    \captionsetup[figure]{font=small, skip=2.5ex}
    \captionsetup[table]{font=small, skip=1ex}
    \captionsetup[subfigure]{font=footnotesize}
    % \captionsetup[subtable]{font=footnotesize}
    \captionsetup{width=.8\linewidth, justification = raggedright}
    % \captionsetup{width=.8\linewidth, justification = centering}
\usepackage{enumitem}                       % enhanced items
\usepackage{lipsum}                         % pseudo texts
\usepackage{setspace}                       % spacing
\usepackage{algorithm, algpseudocode}       % algorithm
    \algrenewcommand{\alglinenumber}[1]{{\scriptsize\bfseries\ttfamily\color{RED}#1}}
\usepackage{footnote}                       % enhanced footnote
\usepackage{listings}						% code listing
	\lstset{
	    basicstyle=\ttfamily\small,     %%% string settings
		stringstyle=\color{RED},
		keywordstyle=\color{BLUE}\bfseries,
		commentstyle=\color{gray},
		tabsize=2,
		breaklines=true,
		showstringspaces=false,
		showspaces=false, 
%			backgroundcolor=\color{gray!4}, 
		    xleftmargin=6pt, 
		    framexleftmargin=6pt,
		    framesep=0pt,
		numberstyle=\bfseries\ttfamily\scriptsize\color{RED},
		numbers=left, % {none, left, right}; position of line number
        numbersep=6pt, % how far the line-numbers are from the code
        stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
			escapeinside={Ω}{≈}
	}

\usepackage{rotating}%\begin{sideways}
			
\usepackage{tikz, xcolor}
	\newcommand*\Circled[1]{% require `tikz`
		\tikz[baseline=(char.base)]{%
			\node[shape=circle, fill=black, inner sep=0.6pt] (char) {%
				\textcolor{white}{\sffamily\bfseries#1}}; }}
				
%\usepackage[scale=.95]{inconsolata}
\PassOptionsToPackage{protrusion, expansion}{microtype} % for better typography

\usepackage{soul}%% \hl{} and \st{}

% for review and revision only, commented out later
\usepackage[yyyymmdd,hhmmss]{datetime}
% \usepackage{fancyhdr}
% \pagestyle{fancy}
% % \thispagestyle{fancy}
% \fancyhf{} % sets both header and footer to nothing
% \renewcommand{\headrulewidth}{0pt}
% \usdate
% % \mmddyydate
% \settimeformat{ampmtime}
% \rhead{\textcolor{gray}{toward another revision; compiled on \sffamily\today\ at \currenttime\ CST}}
% \chead{}
% \lhead{}
% \cfoot{\thepage}
% \newcommand{\changeTo}[1]{{\sffamily\color{RED}#1}}
\newcommand{\changeTo}[1]{#1}

\newcommand{\orderzeroonetwo}{Order-\{0,1,2\}}

\newcommand{\termii}{p\makebox[0.42em]{I}I}
\newcommand{\termpii}{p\makebox[0.42em]{I}I}

\newcommand{\removing}[1]{{\color{gray}#1}}

% \newcommand{\behold}[1]{\hl{#1}}
\newcommand{\behold}[1]{#1}
